Dense Pruning of Pointwise Convolutions in the Frequency Domain

Depthwise separable convolutions and frequency-domain convolutions are two recent ideas for building efficient convolutional neural networks. They are seemingly incompatible: the vast majority of operations in depthwise separable CNNs are in pointwise convolutional layers, but pointwise layers use 1x1 kernels, which do not benefit from frequency transformation. This paper unifies these two ideas by transforming the activations, not the kernels. Our key insights are that 1) pointwise convolutions commute with frequency transformation and thus can be computed in the frequency domain without modification, 2) each channel within a given layer has a different level of sensitivity to frequency domain pruning, and 3) each channel's sensitivity to frequency pruning is approximately monotonic with respect to frequency. We leverage this knowledge by proposing a new technique which wraps each pointwise layer in a discrete cosine transform (DCT) which is truncated to selectively prune coefficients above a given threshold as per the needs of each channel. To learn which frequencies should be pruned from which channels, we introduce a novel learned parameter which specifies each channel's pruning threshold. We add a new regularization term which incentivizes the model to decrease the number of retained frequencies while still maintaining task accuracy. Unlike weight pruning techniques which rely on sparse operators, our contiguous frequency band pruning results in fully dense computation. We apply our technique to MobileNetV2 and in the process reduce computation time by 22% and incur <1% accuracy degradation.

==> sections/methodology_old.tex <==
\section{Methodology}
\label{sec:meth}

This section describes our technique for computing pointwise convolutions in a
DCT-based frequency space, how pruning can be applied in the frequency domain,
and then how this pruning can be learned with standard back-propagation.

\subsection{Pointwise Frequency Domain Convolution}

Our approach to frequency-domain computation is to compress activation data
using a similar approach as JPEG image compression: we divide an activation
tensor into small, fixed-size, square tiles called \emph{macroblocks} and apply
the discrete cosine transform (DCT) to each. The key observation is that running
a 1$\times$1 convolution on this transformed data is equivalent to running it on
the original activation, i.e.:
%
\[ \text{Conv1$\times$1}(X) = \text{DCTinv}( \text{Conv1$\times$1}(
	\text{DCT}( X ))) \]
%
where $X$ is an activation tensor, $\text{DCT}$ is the macroblocked discrete
cosine transform, and $\text{DCT}^{-1}$ is the inverse transformation. This is
possible because the DCT is an invertible linear operator.
Therefore, frequency-domain computation of 1$\times$1 convolutions does not
require frequency-domain training: we can train the entire network normally,
without the transformations, and then insert DCT and inverse DCT ``layers'' to
obtain an equivalent network.

Just like JPEG, our technique is sensitive to macroblock size. Where JPEG uses
macroblocks to localize frequency information to specific locations within the
image, in our setting macroblock size represents a trade-off between the
precision of frequency-domain pruning and the computational overhead from
frequency transformation. Larger macroblocks result in more coefficients per
macroblock wich offers more precision in the frequency space and thus leads to
better pruning potential. On the other hand, the DCT forms the primary overhead
cost for our technique and the computational cost scales quadratically with the
size of the macroblock. In our experiments, we find that 3$\times$3 macroblocks
work well across both networks we evaluate.

We apply the DCT to each channel separately. To implement the DCT, each
macroblock is multiplied by frequency filters (of size $k^2$ where $k$ is the
kernel width) for each coefficient (of which there are $k^2$). With this
implementation of the DCT, the number of required multiply-accumulate operations is:
%
\[
	\text{DCT\_MACs} = c_{in} * \frac{h}{k} * \frac{w}{k} * k^4 = c_{in} * h * w * k^2
\]
%
Processing the same input with a pointwise convolution with a stride of 1 would
require the following operations
%
\[
	\text{Pointwise\_MACs} = c_{in} * h * w * c_{out}
\]
%
To apply the inverse DCT, each coefficient (of which there are $k^2$) is
multiplied by a kernel (of width $k^2$) to transform back to the spatial domain.
%
\[
	\text{IDCT\_MACs} = c_{out} * \frac{h}{k} * \frac{w}{k} * k^4 = c_{out} * h * w * k^2
\]
%
Because our technique transforms to and from the DCT domain for each pointwise
convolution that is pruned, our overhead consists of the operations required to
do this transformation. The ratio of overhead operations to baseline
pointwise operations is the following for each layer:
%
\[
	\frac{\text{DCT\_MACs + IDCT\_MACs}}{\text{Pointwise\_MACs}} = 
	\frac{(c_{in} + c_{out})* k^2}{c_{in} * c_{out}}
\]
%
From the equation above we can see that the larger $c_{in}$ and $c_{out}$ are
the smaller the transformation overhead is with respect to number of baseline
operations. Typically, the number of channels is increased with each subsequent
layer within a CNN and thus the overhead for our technique is less significant
for later layers than earlier layers.

\subsection{Frequency Band Pruning}
\label{sec:pruning}

\begin{figure}
    \centering
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=0.65\linewidth]{figs/pruning-chan.pdf}
        \vspace{-0.5ex}
        \caption{Channel pruning.}
        \label{fig:pruning-chan}
    \end{subfigure}
    \vspace{1ex}
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=0.65\linewidth]{figs/pruning-coeff.pdf}
        \vspace{-0.5ex}
        \caption{Coefficient pruning.}
        \label{fig:pruning-coeff}
    \end{subfigure}
    \vspace{1ex}
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=0.65\linewidth]{figs/pruning-chancoeff.pdf}
        \vspace{-0.5ex}
        \caption{Channel--coefficient pruning.}
        \label{fig:pruning-chancoeff}
    \end{subfigure}
    \vspace{1ex}
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=0.65\linewidth]{figs/pruning-contigband.pdf}
        \vspace{-0.5ex}
        \caption{Channel--frequency band pruning.}
        \label{fig:pruning-contigband}
    \end{subfigure}
    \caption{All pruning strategies for frequency-domain \onebyone{}
	convolutions considered in this paper. The frequency axis is according to
	the output of the 2D DCT, vectorized according to the zigzag pattern
	commonly associated with JPEG~\cite{jpeg}. Each figure depicts a possible pruning mask
	for each technique with 50\% pruning. Gray areas are preserved (nonzero) and
	white areas are pruned (zero).}
	\label{fig:pruning}
\end{figure}

Unlike techniques that use the convolution theorem, transforming activations
with the DCT does not save any computation by itself---its purpose is to enable
pruning in the frequency domain. Before settling on our proposed
pruning technique, channel--frequency band pruning, we evaluated all
alternatives shown in Figure~\ref{fig:pruning}. The first two methods pruned
exclusively in the channel dimension  or in the frequency dimension. These
simple methods offer the least flexibility but serve as relevant baselines. The
most flexible technique is channel--coefficient pruning which prunes arbitrary
frequency coefficients for all channels. The arbitrary nature of this pruning
results in a sparse mask however. As has previously been discussed, sparse
computation is likely to result in poor performance~\cite{yu2017scalpel}. Our
goal is to prune contiguous groups of frequency coefficients, more commonly
referred to as frequency bands. The channel--frequency band pruning technique
enables a large amount of pruning while also enforcing contiguity which enables
fully dense computation.

\paragraph{Channel pruning.}
The method we visualize in Figure~\ref{fig:pruning-chan} removes entire
channels and then sorts them such that all non-zero channels are
contiguous. This technique is equivalent to traditional channel
pruning methods.

\paragraph{Coefficient pruning.}

This approach prunes entire coefficients, independent of the layer's output
channels. Figure~\ref{fig:pruning-coeff} depicts a coefficient pruning mask: all
channels preserve the same set of ``important'' frequencies. Coefficient pruning
can reduce both the cost of the pointwise convolution and the overhead
associated with the DCT and inverse-DCT computations as it is not necessary to
produce frequency coefficients that have been pruned. Our technique
\emph{truncates} the DCT to produce only the unpruned coefficients. While this
approach results in dense computation, it also expresses the incorrect
assumption that all output channels are \emph{equally sensitive} to each
frequency in the activation data. We find that channels are \emph{not} uniformly
sensitive to frequencies in practice, which motivates a more nuanced approach.

\paragraph{Channel--coefficient pruning.}

Channel--coefficient pruning removes the assumption that all channels within a
layer are uniformly sensitive to each frequency. Instead, it acknowledges that
some channels need different frequency information than others. Intuitively,
some channels represent features that require more detail (and hence higher
frequencies) than others. Figure~\ref{fig:pruning-chancoeff} depicts the result:
each channel receives a subset of the frequency coefficients.

We find that this per-channel sensitivity significantly increases the amount of
pruning that is possible for a given accuracy budget. However, the additional
flexibility comes at a cost: the ``random'' effect of the pruning means that the
computation must be sparse. It is not generally possible to reorder channels and
coefficients to pack them into a dense tensor for fast computation.

\paragraph{Channel--frequency band pruning.}

Our final approach extends frequency--coefficient pruning to remove contiguous
ranges of frequencies (bands), thereby recovering dense computation. The key idea relies
on the insight from prior work that CNNs are generally more sensitive to low
frequencies than to high frequencies~\cite{kilian-compress-cnns, deepjpeg,
freq_domain_pruning}. Put differently, coefficient importance is approximately
monotonic with frequency---so if a given coefficient is pruned, all the
higher-frequency coefficients are also likely to be pruned. \emph{Channel--frequency band
pruning} restricts pruning to a contiguous range of the highest frequencies
according to the unique needs of each channel.
Figure~\ref{fig:pruning-contigband} shows a possible mask: each channel
receives a contiguous range of frequencies starting at the lowest frequency.

With this strategy, each channel's computation in the \onebyone{} filter is
dense. We find that this technique prunes nearly the same set of channels as
unrestricted channel--coefficient pruning: significant frequencies naturally
tend to be nearly contiguous. So this technique loses only a few pruned
coefficients while making computation dense and therefore far more efficient.

\subsection{Learned Pruning}

Channel, coefficient, channel--coefficient, and channel--frequency band pruning
each represent different methods for representing coefficient/channel masks, but
how exactly to set the levels for each mask is non-trivial.

Our preliminary experiments rely on activation profiling to determine
which components should be pruned. To profile a network, we perform inference on
training data and record the output activations for each layer. We then average
the absolute magnitude of each frequency coefficient over the training inputs.
The average magnitude represents the importance of a given coefficient to the
network as a whole: coefficients that are small on average are candidates for
pruning. Each pruning technique uses a threshold: they remove components from
the model when their average magnitudes are below this threshold. This
preliminary profiling-based pruning approach is imperfect for two reasons: the
large number of layers makes sweeping all threshold values for all layers
intractable, and also average absolute magnitude may not be the best metric for
evaluating coefficient importance.

To overcome the shortcomings of the profiling-based approach we developed a
new method to learn the best mask for each coefficient using backpropagation.
While any of the different pruning archetypes described above could be learned,
this method is for our recommended pruning technique: channel--frequency band
pruning. We created a new learnable parameter called the \emph{frequency
contiguous mask} (or FCMask) which represents the level of pruning for each
channel while also maintaining frequency contiguity. To apply pruning, each
coefficient in each channel is multiplied by a coefficient mask value derived from
the FCMask value for that channel.

\begin{figure} \centering
	\includegraphics[width=0.6\linewidth]{figs/learned_freqcontigmask.pdf}%
	\caption{Here we graph how each individual coefficient's mask is a
	function of FCMask. This example is for four coefficients, which would
	correspond to a 2$\times$2 macroblock}
	\label{fig:learned_freqcontigmask}
\end{figure}
%
\begin{equation*}\label{eq:FCMask_coefmask}
  \begin{aligned}
	  m &= \text{num\_coefs} = \text{macrobock\_width}^{2} \\
	  \text{coefmask_n} &= (\text{FCMask} - \frac{n}{m}) \times m
  \end{aligned}
\end{equation*}
%\text{coefmask_n} &= (\text{FCMask} - \frac{n}{\text{num\_coefs}}) \times \text{num\_coefs}
 the masks for each coefficient, As shown in Figure~\ref{fig:learned_freqcontigmask} and the equation above, when
FCMask is set to 0.0 all coefficient masks in the channel are equal to 0.0
(removing all data from the channel entirely) and when FCMask is set to 1.0 all
frequency masks are equal to 1.0 (no pruning is applied). FCMasks are
initialized to 1.0 and are influenced to decrease by our modified loss function.
Consider the case where a channel's FCMask gradient decreases the value of
FCMask from 1.0 to 0.9. Coefficient masks 0-2 will remain at 1.0, but frequency
mask 3 will slightly decrease in value. Because during inference each
coefficient value is multiplied by its corresponding coefficient mask, the
decrease in the coefficient mask will decrease the impact that this individual
coefficient has on the network as a whole. It is this ability to make small
adjustments to the impact of each coefficient that enables this learning
technique to succeed, since rounding all masks to 0 or 1 during training would
prevent gradients from propagating through the network. After training is
completed, all coefficient masks are rounded and fixed to 0 or 1 so that we can
save on computation.

The modified loss function which influences FCMask values to be decreased can be seen below:
%
$$
\text{loss} = \text{cross\_entropy} + \lambda \times \sum_{l=0}^{num\_layers} avg(|FCMask_{l}|)
$$
%
We preserve a cross entropy loss component to maintain the accuracy of the
classification task that our model is trained for. We also introduce a new
metaparameter, $\lambda$, to control the degree of impact that the new loss
component will have on the network as a whole. The primary regularization value
in this loss function is a sum taken over all layers of the average absolute
value for FCMasks over all channels in each layer. Smaller FCMask values
decrease the loss function and are thus rewarded. On the other hand, masking
coefficients may increase the cross entropy if these coefficients are important
to the network. We have intentionally built in this tension into the loss
function to achieve a balance between efficiency and accuracy.

%\begin{figure}
%    \centering
%    \begin{subfigure}[b]{0.45\linewidth}
%        \centering
%        \includegraphics[width=\linewidth]{figs/module.features.2.conv.6.tforminv_mask.freqcontig_mask.pdf}%
%        \caption{Pointwise in Block 2}
%        \label{fig:learned_freqcontigmask_example2}
%    \end{subfigure}
%    \hspace{1ex}
%    \begin{subfigure}[b]{0.45\linewidth}
%        \centering
%        \includegraphics[width=\linewidth]{figs/module.features.10.conv.0.tforminv_mask.freqcontig_mask.pdf}%
%        \caption{Pointwise in Block 10}
%        \label{fig:learned_freqcontigmask_example10}
%    \end{subfigure}
%    \caption{Examples of learned contiguous frequency band masks in MobileNet v2 }
%    \label{fig:learned_freqcontigmask_examples}
%\end{figure}


\begin{figure}
    \centering
        \includegraphics[width=\linewidth]{figs/module.features.10.conv.0.tforminv_mask.freqcontig_mask.pdf}%
    \caption{FCMask values for all channels in the first pointwise layer of Block
	10 of \mobilenet, using a 3$\times$3 macroblock size. The horizontal lines
	demarcate the regions of FCMask values which pertain to each of the nine
	coefficients.}
    \label{fig:learned_freqcontigmask_example}
\end{figure}

Figure~\ref{fig:learned_freqcontigmask_example} shows an example of a learned
frequency contiguous mask for MobileNet v2 when trained on ImageNet. The
heterogeneous sensitivity of each channel to frequency can be observed as there
is significant variation in the value of FCMask for each channel.
Figure~\ref{fig:learned_freqcontigmask_example} shows that this layer has has
pruned away the highest frequency coefficient for all channels, and has
also pruned all coefficients for as subset of channels.

\subsection{Dense Frequency-Domain Computation}

The primary motivation for our pruning technique over traditional pruning is
that our method enables dense computation while still requiring fewer operations
than an unpruned convolution. Figure \ref{fig:dense_compute} (a) shows a
standard pointwise \onebyone layer, and (b) shows a mathematically equivalent
operation which applies the DCT before and IDCT after the pointwise operation.
The DCT and IDCT masks in Figure \ref{fig:dense_compute} (b) shows that not all coefficients are
needed for all channels, but (b) would require expensive sparse computation to
avoid computing the pruned coefficients.

Figure~\ref{fig:dense_compute} (c) shows our proposal: group coefficients into
frequency bands and then compute the pointwise convolution on each frequency
band separately. The baseline pointwise convolution would
need to multiply all weights by all coefficients in each input channel to
produce all coefficients for all output channels. In contrast,
dividing the computation into frequency bands offers the ability to only process
the channels that pertain to the frequency band of interest. In the example
shown in Figure \ref{fig:dense_compute} (c), frequency band 0 only has non-zero
coefficients from channels $c_0-c_y$ at the input, and only produces non-zero
output for channels $\hat{c}_0-\hat{c}_y$. Similarly, frequency band 1 only has non-zero
coefficients from channels $c_0-c_x$ at the input, and only produces non-zero
output for channels $\hat{c}_0-\hat{c}_x$. By reducing the total volume of input
and output data for each pointwise convolution we have saved a significant
amount of computation while remaining entirely dense.

\begin{figure} \centering
	\includegraphics[width=0.8\linewidth]{figs/dense_compute.pdf}%
	\caption{Three equivalent pointwise convolutions:
	typical, frequency domain, separate frequency bands}
	\label{fig:dense_compute}
\end{figure}

%\begin{figure} \centering
%	\includegraphics[width=0.8\linewidth]{figs/quantized_fbands.png}%
%	\caption{Quantizing Channel-Specific Masks Into Frequency Band Masks}
%	\label{fig:quantfband}
%\end{figure}

%\subsection{Interleaving Transforms into the Network}

%\begin{figure}
%    \centering
%    \begin{subfigure}[b]{0.45\linewidth}
%        \centering
%        \includegraphics[width=\linewidth]{figs/freq_domain_mobilenetv2-flat.pdf}%
%        \caption{\mobilenet~\cite{mobilenetv2} block.}
%        \label{fig:mobilenetv2_block}
%    \end{subfigure}
%    \hspace{1ex}
%    \begin{subfigure}[b]{0.45\linewidth}
%        \centering
%        \includegraphics[width=\linewidth]{figs/freq_domain_resnext-flat.pdf}%
%        \caption{\resnext~\cite{resnext} block.}
%        \label{fig:resnext_block}
%    \end{subfigure}
%    \caption{Residual blocks for two CNN architectures with the 1$\times$1 convolution computed in the frequency domain. Shading indicates frequency-domain computation.}
%    \label{fig:layers}
%\end{figure}
%
%To make our pruning approach work in the context of CNNs, we need to
%integrate our DCT and inverse DCT layers into existing network architectures.
%This section shows how to integrate the transform into two depthwise separable
%CNNs with subtle differences: \mobilenet~\cite{mobilenetv2} and
%\resnext~\cite{resnext}.
%
%Both architectures organize their layers into repeating \emph{residual blocks}.
%Figure~\ref{fig:layers} shows one such block for each architecture. In both networks,
%each block has two 1$\times$1 convolutions and one 3$\times$3 convolution. In
%\mobilenet, the output of the final 1$\times$1 convolution feeds through a batch
%normalization step and a residual connection into the next block's first
%1$\times$1 layer. As Figure~\ref{fig:mobilenetv2_block} shows, this structure
%allows us to use only a single DCT/DCT$^-1$ pair for the entire block.

%In \resnext, however, the 1$\times$1 layers for two adjacent blocks are
%separated by the ReLU layer. Unlike the linear 1$\times$1 layer, computing this
%nonlinearity in the frequency domain is \emph{not} equivalent to computing it on
%the original, untransformed activation. And in our experiments, doing so yields
%a significant accuracy loss: CIFAR-10 accuracy in \resnext drops from 95.75\% to
%93.78\% when computing the ReLU in the frequency domain, while removing it
%altogether yields 94.43\% accuracy. (We also tried computing the ReLU only on
%the DC component of the frequency-domain data, but the accuracy still dropped to
%95.01\%.) Figure~\ref{fig:resnext_block} shows how to insert \emph{two}
%DCT/inverse-DCT pairs into \resnext, with one around each 1$\times$1 layer and
%with all ReLUs computed on untransformed inputs. As we find in
%Section~\ref{sec:eval:resnext}, the additional overhead from doubling the
%transformations does not result in significant performance cost.

